CVA6 RISC-V Virtualization: Architecture, Microarchitecture, and Design Space Exploration

Virtualization is a key technology used in a wide range of applications, from cloud computing to embedded systems. Over the last few years, mainstream computer architectures were extended with hardware virtualization support, giving rise to a set of virtualization technologies (e.g., Intel VT, Arm VE) that are now proliferating in modern processors and SoCs. In this article, we describe our work on hardware virtualization support in the RISC-V CVA6 core. Our contribution is multifold and encompasses architecture, microarchitecture, and design space exploration. In particular, we highlight the design of a set of microarchitectural enhancements (i.e., G-Stage Translation Lookaside Buffer (GTLB), L2 TLB) to alleviate the virtualization performance overhead. We also perform a Design Space Exploration (DSE) and accompanying post-layout simulations (based on 22nm FDX technology) to assess Performance, Power ,and Area (PPA). Further, we map design variants on an FPGA platform (Genesys 2) to assess the functional performance-area trade-off. Based on the DSE, we select an optimal design point for the CVA6 with hardware virtualization support. For this optimal hardware configuration, we collected functional performance results by running the MiBench benchmark on Linux atop Bao hypervisor for a single-core configuration. We observed a performance speedup of up to 16% (approx. 12.5% on average) compared with virtualization-aware non-optimized design at the minimal cost of 0.78% in area and 0.33% in power. Finally, all work described in this article is publicly available and open-sourced for the community to further evaluate additional design configurations and software stacks.

==> Guidelines/general_guides.tex <==

% General guidelines:
% 1. The maximum length of each manuscript is 14 pages for a regular paper and 5 pages for a brief including references, figures, tables, equations and biographies. Submitted papers that are not compliant with either the allowed page lengths or the style format will be returned to the authors. The biographies and photographs are now optional.
% 2. Each manuscript should be complete with illustrations (if any), abstract, and at least 5 keywords. The abstract must be a concise yet comprehensive reflection of what is in the article. In particular:
%
%    2.1 The abstract must be self-contained, without abbreviations, footnotes, or references. It should be a microcosm of the full article.
%    2.2 The abstract must be between 100-250 words. Be sure to adhere to these limits; otherwise, it must be edited accordingly.
%    2.3 The abstract must be written as one paragraph, and should not contain displayed mathematical equations or tabular material.
%    2.4 The abstract should include three or four different keywords or phrases, as this will help readers to find it. It is important to avoid over-repetition of such phrases as this can result in a page being rejected by search engines.
%    2.5 Ensure that the abstract reads well and is grammatically correct.
%
% 3. Each manuscript should contain in the first page the full names and (typically as footnotes) affiliation of all authors, as well as their email addresses. Acknowledgement of financial support is often placed at the end of the footnote.
% 4. References should appear in a separate bibliography section at the end of the paper, with items referred to by numerals in square brackets, e.g., [12]. In either case, references should be complete and in IEEE style. Important: If part of the manuscript has been presented, published or submitted elsewhere, this should be noted in the submission form that the author will access before uploading their manuscript. In particular, authors must explain major differences between the prior work(s) and the manuscript submitted to this TRANSACTIONS. This must be attached at the end of the manuscript. This should also be noted in the first paragraph of the first footnote.

